BYOL-S: Learning Self-supervised Speech Representations by Bootstrapping

Methods for extracting audio and speech features have been studied since pioneering work on spectrum analysis decades ago. Recent efforts are guided by the ambition to develop general-purpose audio representations. For example, deep neural networks can extract optimal embeddings if they are trained on large audio datasets. This work extends existing methods based on self-supervised learning by bootstrapping, proposes various encoder architectures, and explores the effects of using different pre-training datasets. Lastly, we present a novel training framework to come up with a hybrid audio representation, which combines handcrafted and data-driven learned audio features. All the proposed representations were evaluated within the HEAR NeurIPS 2021 challenge for auditory scene classification and timestamp detection tasks. Our results indicate that the hybrid model with a convolutional transformer as the encoder yields superior performance in most HEAR challenge tasks.

==> drafts/Methods_embeddings.tex <==
% Referring to the downstream tasks from the previous section, the embeddings generated for the tasks were either generated from the entire audio sample (Scene Embeddings, Table~\ref{tab:scene_datasets}) or by breaking the sample down to chunks of fixed sizes and generate window representations with their corresponding timestamps (Timestamp Embeddings). Two tasks required timestamp embeddings (DCASE and MAESTRO). Accordingly, we separated them from the rest of the tasks as shown in Table \ref{tab:timestamp_data}. Also, the results are demonstrated separately (section~\ref{sec:res_timestamps}) to give space for exploring the timestamp hyperparameters; window and hop sizes.


==> drafts/Methods_hear_sub.tex <==
% Our early submission to the challenge was BYOL-S, a speech-specific version of BYOL-A~\citep{niizumi2021byol} which yielded competitive results across the provided datasets. In particular, BYOL-S was among the best performers in speech emotion recognition (CREMA-D~\citep{cao2014crema}), music vs. speech classification (GTZAN~\citep{tzanetakis2002musical}) and speaker count (Libricount~\citep{stoter2018libricount}).

% In addition to this submission, we evaluated different versions of BYOL-S by assessing different pre-training setups, encoder architectures, tuning several hyperparameters, as well as the "hybrid" version presented in Sec.~\ref{sec:hybrid}.

==> drafts/Table1113.tex <==
\begin{table}[h!]
\small
\centering
\vspace{-0.3cm}
\caption{Top-1 accuracy of encoder-based variants of BYOL-S on speech-related tasks. All HEAR baselines were achieved using wav2vec2.}
\begin{tabular}{lccccccc}
\toprule
        & \rotatebox{90}{CREMA-D} 
        & \rotatebox{90}{LibriCount} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
        & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
        & \rotatebox{90}{VoxLingua} 
        & \rotatebox{90}{Average} \\
\midrule
HEAR & 65.6 & 69.2 & 87.9 & 83.8 & 6.8 & \textsb{49.3} & 59.3 \\
\midrule
Default           &     \textsb{66.4}     & 78.6 & \textsb{92.6}    & \textsb{94.3}              & 15.1           & 41.2 & \textsb{64.7}          \\
Resnetish-34 & 63.5 & 77.0           & 83.2    & 88.9              & 14.8           & 35.8 & 60.5         \\
CLSTM       & 64.0 & 78.1 & 91.3    & 92.5   & \textsb{16.0}   & 24.3 & 61.0  \\
CvT          & \textsb{66.4}          & \textsb{84.8}          & 92.0     & 93.1              & \textsb{16.2}           & 37.0 & \textsb{64.9}\\
\bottomrule
\end{tabular}
\label{tab:encoder_results_speech}\vspace{-0.3cm}
\end{table}


\begin{table}[h!]
\small
\centering
\caption{Comparison of encoder architectures on environmental sound-related datasets. Top-1 accuracy was used for each dataset but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2. $^*$: \textit{task not completed due to exhausting GPU memory}.}
 \begin{tabular}{lccccc}
    \toprule
    \begin{tabular}{@{}l@{}}BYOL-S \\ Encoder\end{tabular}  & \rotatebox{90}{Beehive states} & \rotatebox{90}{ESC} & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       & \rotatebox{90}{Average}\\
    \midrule
     HEAR & 53.5$^\sharp$ & 56.1$^\dagger$ & 34.2$^\dagger$ & 86.3$^\sharp$ & 57.5\\ 
    \midrule
     Default &  52.8 & \textsb{81.9} & \textsb{49.9} & \textsb{96.4} & \textsb{70.3 }\\
     Resnetish-34 & 52.8  & 71.5 & 43.3 & 86.3 & 63.5 \\
     CLSTM &  51.4 & 73.9 & 39.4 & 86.9 & 62.9 \\
     CvT & -$^*$ & 79.9 & 48.3 & 89.3 & -\\
     \bottomrule
 \end{tabular}
\label{tab:encoder_results_env}\vspace{-0.3cm}
\end{table}
\setlength{\tabcolsep}{6pt}


\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
    \small
    \centering
    
    \caption{Top-1 accuracy of encoder-based variants of BYOL-S on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    
    \begin{NiceTabular}{l@{\hspace{10pt}}c@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}c}
    
    \toprule
    BYOL-S & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
    Encoder  & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
    
    \midrule
    HEAR & 92.8$^\sharp$ & 78.0$^\dagger$ & 94.6$^\dagger$ & 94.3$^\dagger$ & 82.8$^\dagger$ & \textsb{87.0}$^\sharp$ & \textsb{92.6}$^\sharp$ & \textsb{90.0}$^\sharp$ & \textsb{95.7}$^\sharp$ & \textsb{89.8} \\
    \midrule
    
    Default  & 91.1 & \textsb{83.8} & 92.3 & \textsb{97.3} & 92.9 & 42.0 & 44.0 & 70.0 & 73.4 & 76.3 \\
    Resnetish-34 & 92.4 & 77.4 & 96.9 & 96.1  & 88.7 & 26.0 & 22.4 & 44.9 & 47.4 & 65.8 \\
    CLSTM & \textsb{97.0} & 75.9 & 96.2 & 96.7 & 89.7 & 28.6 & 32.0 & 57.6 & 65.0 & 71.0 \\
    CvT & 96.2 & \textsb{84.2} & \textsb{97.7} & \textsb{97.5} & \textsb{94.0} & 53.0 & 55.2 & 76.1 & 85.0 & 82.1 \\
    \bottomrule
    
    \end{NiceTabular}
      
    \label{tab:encoder_results_music}\vspace{-0.3cm}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/Table1416.tex <==
\begin{table}[h!]
    \small
    \centering
    \vspace{-0.34cm}
    \caption{Top-1 accuracy of hybrid BYOL-S variants on speech-related tasks. All HEAR baselines were achieved using wav2vec2.}\vspace{4pt}
    \begin{tabular}{l*7{c}}
    \toprule
    & \rotatebox{90}{CREMA-D} 
    & \rotatebox{90}{LibriCount} 
    & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
    & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
    & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
    & \rotatebox{90}{VoxLingua} 
    & \rotatebox{90}{Average} \\
    \midrule
    HEAR & 65.6 & 69.2 & 87.9 & 83.8 & 6.8 & \textsb{49.3} & 59.3 \\
\midrule
     BYOL-S & 66.4  & \textsb{92.6} & 94.3 & 78.6 & 15.1 & 41.2 & 64.7   \\
     Hybrid BYOL-S &  66.1 & 91.6 & 93.8 & 81.6 & 14.2 & 43.8 & 65.2  \\
     BYOL-S, CvT &  66.4 & 92.0 & 93.1 & \textsb{84.8} & \textsb{16.2} & 37.0 & 64.9 \\
     Hybrid BYOL-S,  CvT & \textsb{67.2} & \textsb{92.6} & \textsb{95.8} & 83.5 & \textsb{16.3} & 42.2 & \textsb{66.3} \\
     \bottomrule
      \end{tabular}
  \label{tab:hybrid_speech}\vspace{-0.34cm}
\end{table}

\setlength{\tabcolsep}{6pt}
\begin{table}[h!]
    \small
    \centering
    \caption{Performance of hybrid BYOL-S on environment sound-related tasks. Top-1 accuracy was used for each task but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2. $^*$: \textit{task not completed due to exhausting GPU memory}}
    \begin{tabular}{l@{\hspace{20pt}}cccc@{\hspace{20pt}}c}
    \toprule
            & \rotatebox{90}{Beehive states} & \rotatebox{90}{ESC} & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       & \rotatebox{90}{Average}\\
    \midrule
     HEAR & 53.5$^\sharp$ & 56.1$^\dagger$ & 34.2$^\dagger$ & 86.3$^\sharp$ & 57.5\\ 
    \midrule
    BYOL-S            & 52.8 & 81.9 & 49.9 & \textsb{96.4} & \textsb{70.3} \\
    Hybrid BYOL-S     & \textsb{53.0}  & 82.4 & 48.9 & 95.2 & \textsb{69.9} \\
    BYOL-S/CvT        & -$^*$   & 79.9 & 48.3 & 89.3 & - \\
    Hybrid BYOL-S/CvT & -$^*$  & \textsb{83.8} & \textsb{52.0} & \textsb{96.4} & -\\
    \bottomrule
    \end{tabular}
    \label{tab:hybrid_env}\vspace{-0.34cm}
\end{table}
\setlength{\tabcolsep}{6pt}


\setlength{\tabcolsep}{2.5pt}
\begin{table}[h!]
\small
\centering
\caption{Top-1 accuracy of hybrid variants of BYOL-S on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}\vspace{4pt}
    \begin{NiceTabular}{l@{\hspace{8pt}}c@{\hspace{8pt}}*{2}{c}@{\hspace{8pt}}*{2}{c}@{\hspace{8pt}}*{2}{c}@{\hspace{8pt}}*{2}{c}@{\hspace{8pt}}c}
    \toprule
    & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
    & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
    \midrule
     HEAR & 92.8$^\sharp$ & 78.0$^\dagger$ & 94.6$^\dagger$ & 94.3$^\dagger$ & 82.8$^\dagger$ & \textsb{87.0}$^\sharp$ & \textsb{92.6}$^\sharp$ & \textsb{90.0}$^\sharp$ & \textsb{95.7}$^\sharp$ & \textsb{89.8} \\
     \midrule
     BYOL-S            & 91.1 & 83.8 & 92.3 & \textsb{97.5} & 93.2 & 42.0  & 44.0  & 70.0   & 73.4 & 76.4 \\
Hybrid BYOL-S      & 92.8 & \textsb{85.9} & 96.9 & 96.1 & 88.7 & 35.8 & 38.0  & 71.1 & 75.0 & 75.6  \\
BYOL-S/CvT        & \textsb{96.2} & 84.2 & \textsb{97.7} & \textsb{97.5} & 94.0 & 53.0  & 55.2 & 76.1 & 85.0 & 82.1 \\
Hybrid BYOL-S/CvT & 94.5 & \textsb{85.8} & 96.2 & \textsb{97.7} & \textsb{94.9} & 56.8 & 59.2 & 79.5 & 83.0 & 83.1  \\
    \bottomrule
  \end{NiceTabular}
  \label{tab:hybrid_music}\vspace{-0.3cm}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/Table1719.tex <==
\begin{table}[h!]
    \small
    \centering
    \vspace{-0.34cm}
    \caption{Top-1 accuracy of hybrid BYOL-S with different loss weights on speech-related tasks. All HEAR baselines were achieved using wav2vec2.}
        \begin{tabular}{l@{\hspace{20pt}}cccccc@{\hspace{20pt}}c}
        \toprule
            \begin{tabular}{@{}l@{}}Hybrid BYOL-S/CvT \\ $\alpha$:$\beta$ \end{tabular}
            & \rotatebox{90}{CREMA-D} 
            & \rotatebox{90}{LibriCount} 
            & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
            & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
            & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
            & \rotatebox{90}{VoxLingua} 
            & \rotatebox{90}{Average} \\
        \midrule
    % HEAR/crepe & 36.2 & 49.9 & 16.8 & 19.6 & 5.1 & 15.1 & 23.8 \\
    HEAR & 65.7 & 67.6 & 79.7 & 88.5 & 7.2 & \textsb{49.7} & 59.7 \\
    \midrule
    1:4 & 62.9          & \textsb{84.4} & 86.2          & 90.7          & 12.0          & 27.1 & 60.6\\
    1:2 & 64.4          & 83.5          & 89.6          & 92.7          & 13.6          & 35.3 & 63.2\\
    2:3 & 66.0          & \textsb{84.1} & 91.9          & 93.8          & 14.6          & 38.7 & 64.9\\
    1:1 & \textsb{67.2} & 83.5          & \textsb{92.6} & \textsb{95.8} & \textsb{16.3} & 42.2 & \textsb{66.3}\\
    3:2 & \textsb{66.7} & 82.7          & 92.5          & 94.8          & 15.2          & 34.0 & 64.3\\
    2:1 & 65.8          & 81.2          & \textsb{92.7} & 94.7          & \textsb{15.8} & 39.8 & 65.0\\
    4:1 & 66.5          & 80.6          & \textsb{93.1} & 94.6          & \textsb{16.2} & 38.0 & 64.8\\
        \bottomrule
        \end{tabular}
        \label{tab:hybrid_weights_speech}\vspace{-0.25cm}
\end{table}

\begin{table}[h!]
    \small
    \centering
    \vspace{-4pt}
    \caption{Performance of hybrid BYOL-S with different loss weights on environmental sound-related datasets. Top-1 accuracy was used for each dataset but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2. $^*$: \textit{task not completed due to exhausting GPU memory}}
    \begin{tabular}{l@{\hspace{20pt}}cccc@{\hspace{20pt}}c}
    \toprule
            \begin{tabular}{@{}l@{}}Hybrid BYOL-S/CvT \\ $\alpha$:$\beta$ \end{tabular}
            & \rotatebox{90}{Beehive states} 
            & \rotatebox{90}{ESC} 
            & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       
            & \rotatebox{90}{Average}\\
    \midrule
% HEAR/crepe & -$^*$ & 29.4 & 15.9 & 91.7 & 45.7\\
% HEAR/wav2vec2 & -$^*$ & 59.2 & 34.6$ & 77.1 & 57.0\\
HEAR & -$^*$ & 59.2$^\dagger$ & 34.6$^\dagger$ & 91.7$^\sharp$& 61.8 \\
     \midrule
1:4 & -$^*$ & 72.5          & 42.7          & 88.7          & 68.0\\
1:2 & -$^*$ & 78.4          & 46.1          & 90.5          & 71.7\\
2:3 & -$^*$ & 79.6          & 47.8          & 96.4          & 74.6\\
1:1 & -$^*$ & \textsb{83.8} & \textsb{50.2} & 96.4          & \textsb{76.8}\\
3:2 & -$^*$ & 82.3          & 47.9          & \textsb{97.6} & 75.9\\
2:1 & -$^*$ & 83.1          & 48.3          & 95.8          & 75.7\\
4:1 & -$^*$ & 82.4          & 48.7          & 94.0          & 75.0\\
     \bottomrule
  \end{tabular}
  \label{tab:hybrid_weights_env}\vspace{-0.25cm}
\end{table}


\setlength{\tabcolsep}{3pt} 
\begin{table}[!htb]
    \small
    \centering
    \vspace{-4pt}
    \caption{Top-1 accuracy of Hybrid BYOL-S with different loss weights on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    \begin{NiceTabular}{l@{\hspace{10pt}}c@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}c}
    \toprule
    \begin{tabular}{@{}l@{}}Hybrid BYOL-S/CvT \\ $\alpha$:$\beta$ \end{tabular}
    & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
    & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
    \midrule
% HEAR/crepe & 93.2 & 64.5 & 86.7 & 88.7 & 82.3 & \textsb{87.2} & \textsb{93.4} & \textsb{89.5} & \textsb{95.2} & \textsb{86.7} \\
% HEAR/wav2vec2 & 89.4 & 78.0 & 92.3 & 94.7 & 82.8 & 40.0 & 44.6 & 66.7 & 71.9 & 73.4 \\
HEAR & 93.2$^\sharp$ & 78.0$^\dagger$ & 92.3$^\dagger$ & 94.7$^\dagger$ & 82.8$^\dagger$ & \textsb{87.2}$^\sharp$ & \textsb{93.4}$^\sharp$ & \textsb{89.5}$^\sharp$ & \textsb{95.2}$^\sharp$ & \textsb{89.6} \\
     \midrule
1:4 & 94.9 & 82.2 & 95.3 & 97.2 & 96.0 & 66.4 & 68.6 & 80.8 & 84.6 & 85.1\\
1:2 & \textsb{96.2} & 84.8 & 94.6 & \textsb{97.6} & \textsb{96.7} & 65.4 & 69.6 & 81.6 & 85.8 & 85.8\\
2:3 & 93.2 & 86.1 & 93.8 & \textsb{97.5} & \textsb{96.6} & 67.0 & 69.8 & 81.1 & 85.4 & 85.6\\
1:1 & 94.5 & 85.8 & \textsb{96.2} & \textsb{97.7} & 94.9 & 56.8 & 59.2 & 79.5 & 83.0 & 83.1\\
3:2 & \textsb{95.8} & 85.6 & 94.6 & \textsb{97.7} & \textsb{96.7} & 64.0 & 67.0 & 81.9 & 85.9 & 85.5\\
2:1 & 94.9 & \textsb{86.4} & 94.6 & \textsb{97.8} & \textsb{96.6} & 62.8 & 66.4 & 80.9 & 85.0 & 85.0\\
4:1 & 94.9 & \textsb{86.8} & 92.3 & \textsb{97.8} & \textsb{96.4} & 63.2 & 65.6 & 79.9 & 84.3 & 84.6\\
     \bottomrule
    \end{NiceTabular}
    \label{tab:hybrid_weights_music}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/Table2022.tex <==
\begin{table}[h!]
\small
\centering
\caption{Top-1 accuracy of openSMILE and BYOL-S features with different ensemble approaches on speech-related tasks. All HEAR baselines were achieved using crepe and wav2vec2.}
    \begin{tabular}{l@{\hspace{20pt}}cccccc@{\hspace{20pt}}c}
    \toprule
        \begin{tabular}{@{}l@{}}\end{tabular}
        & \rotatebox{90}{CREMA-D} 
        & \rotatebox{90}{LibriCount} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
        & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
        & \rotatebox{90}{VoxLingua} 
        & \rotatebox{90}{Average} \\
    \midrule
HEAR & 65.6 & 69.2 & 87.9 & 83.8 & 6.8 & \textsb{49.3} & 59.3 \\
\midrule
OS & 21.6 & 19.0 & 8.3 & 14.1 & & 9.7 & \\
BYOL-S/CvT & 66.4 & \textsb{84.8} & 92.0 & 93.1 & \textsb{16.2} & 37.0 & 64.9 \\
BYOL-S/CvT + OS & 21.7 & 20.7 & 8.3 & 14.9 & & 9.7 & \\
Hybrid BYOL-S/CvT & \textsb{67.2} & 83.5          & \textsb{92.6} & \textsb{95.8} & \textsb{16.3} & 42.2 & \textsb{66.3}\\
    \bottomrule
    \end{tabular}
    \label{tab:ensemble_speech}\vspace{-0.25cm}
\end{table}

\begin{table}[h!]
    \small
    \centering
    \caption{Performance of openSMILE and BYOL-S features with different ensemble approaches on environmental sound-related datasets. Top-1 accuracy was used for each dataset but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    \begin{tabular}{l@{\hspace{20pt}}cccc@{\hspace{20pt}}c}
    \toprule
            \begin{tabular}{@{}l@{}}\end{tabular}
            & \rotatebox{90}{Beehive states} 
            & \rotatebox{90}{ESC} 
            & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       
            & \rotatebox{90}{Average}\\
    \midrule
     HEAR & 53.5$^\sharp$ & 56.1$^\dagger$ & 15.9$^\sharp$ & 86.3$^\sharp$ & 53.0\\ 
     \midrule
OS                & -$^*$ & 6.2 & 5.3 & 39.3 & 16.9\\
BYOL-S/CvT        & -$^*$ & 79.9 & 48.3 & 89.3 & 72.5\\
BYOL-S/CvT + OS   & -$^*$ & 6.3 & 5.3 & 41.2 & 17.6\\
Hybrid BYOL-S/CvT & -$^*$ & \textsb{83.8} & \textsb{50.2} & \textsb{96.4} & \textsb{76.8}\\
     \bottomrule
  \end{tabular}
  \label{tab:ensemble_env}\vspace{-0.25cm}
\end{table}
\setlength{\tabcolsep}{3pt}


\begin{table}[!htb]
    \small
    \centering
    \caption{Top-1 accuracy of openSMILE and BYOL-S features with different ensemble approaches on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    \begin{NiceTabular}{l@{\hspace{10pt}}c@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}c}
    \toprule
    \begin{tabular}{@{}l@{}}\end{tabular}
    & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
    & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
    \midrule
     HEAR & 92.8$^\sharp$ & 78.0$^\dagger$ & 94.6$^\dagger$ & 94.3$^\dagger$ & 82.8$^\dagger$ & \textsb{87.0}$^\sharp$ & \textsb{92.6}$^\sharp$ & \textsb{90.0}$^\sharp$ & \textsb{95.7}$^\sharp$ & \textsb{89.8} \\
    \midrule
    OS                & 41.5 & 26.9 & 78.3 & 32.2 & 22.1 & 1.6 & 8.2 & 1.7 & 8.5 & 24.6\\
    BYOL-S/CvT        & \textsb{96.2} & 84.2 & \textsb{97.7} & \textsb{97.5} & 94.0 & 53.0 & 55.2 & 76.1 & 85.0 & 82.1\\
    BYOL-S/CvT + OS   & 52.1 & 24.6 & 79.7 & 32.1 & 21.9 & 0.8 & 9.0 & 1.7 & 8.5 & 25.6\\
    Hybrid BYOL-S/CvT & 94.5 & \textsb{85.8} & 96.2 & \textsb{97.7} & \textsb{94.9} & 56.8 & 59.2 & 79.5 & 83.0 & 83.1\\
     \bottomrule
    \end{NiceTabular}
    \label{tab:ensemble_music}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/Table47.tex <==
\begin{table}[h!]
\small
\centering
\caption{Top-1 accuracy of BYOL-A, BYOL-S and BYOL-S\texttt{++} on speech-related tasks. All HEAR baselines were achieved using wav2vec2.}
    \begin{tabular}{l@{\hspace{20pt}}cccccc@{\hspace{20pt}}c}
    \toprule
        & \rotatebox{90}{CREMA-D} 
        & \rotatebox{90}{LibriCount} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
        & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
        & \rotatebox{90}{VoxLingua} 
        & \rotatebox{90}{Average} \\
    \midrule
HEAR & 65.6 & 69.2 & 87.9 & 83.8 & 6.8 & \textsb{49.3} & 59.3 \\
\midrule
BYOL-A            & 62.3          & 78.8        & 89.6 & 92.4 & 13.7          & 39.0          & 62.6 \\
BYOL-S            & \textsb{66.4} & 78.5        & 92.6          & 94.3 & \textsb{15.1}          & 41.2          & 64.7 \\
BYOL-S\texttt{++} & \textsb{66.4} & \textsb{80.0} & \textsb{93.2} & \textsb{95.0}  & \textsb{15.4} & 47.8 & \textsb{66.3} \\
    \bottomrule
    \end{tabular}
    \label{tab:pretraining_results_speech}\vspace{-0.25cm}
\end{table}
\begin{table}[h!]
    \small
    \centering
    \caption{Performance of BYOL-A, BYOL-S and BYOL-S\texttt{++} variants on environmental sound-related datasets. Top-1 accuracy was used for each dataset but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    \begin{tabular}{l@{\hspace{20pt}}cccc@{\hspace{20pt}}c}
    \toprule
            & \rotatebox{90}{Beehive states} 
            & \rotatebox{90}{ESC} 
            & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       
            & \rotatebox{90}{Average}\\
    \midrule
     HEAR & 53.5$^\sharp$ & 56.1$^\dagger$ & 34.2$^\dagger$ & 86.3$^\sharp$ & 57.5\\ 
     \midrule
     BYOL-A            & 48.8          & 78.9          & 48.9          & 87.5          & 66.0          \\
     
     BYOL-S            & 52.8 & \textsb{81.9} & \textsb{49.9} & \textsb{96.4} & \textsb{73.0} \\
     
     BYOL-S\texttt{++} & \textsb{55.0}          & 80.0            & \textsb{49.4}          & 92.9          & 68.2 \\
     \bottomrule
  \end{tabular}
  \label{tab:pretraining_results_env}\vspace{-0.25cm}
\end{table}
\setlength{\tabcolsep}{3pt}
\begin{table}[!htb]
    \small
    \centering
    \caption{Top-1 accuracy on BYOL-A, BYOL-S, and BYOL-S\texttt{++} on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
    \begin{NiceTabular}{l@{\hspace{10pt}}c@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}c}
    \toprule
    & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
    & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
    \midrule
     HEAR & 92.8$^\sharp$ & 78.0$^\dagger$ & 94.6$^\dagger$ & 94.3$^\dagger$ & 82.8$^\dagger$ & \textsb{87.0}$^\sharp$ & \textsb{92.6}$^\sharp$ & \textsb{90.0}$^\sharp$ & \textsb{95.7}$^\sharp$ & \textsb{89.8} \\
     \midrule
     BYOL-A   & 91.9 & \textsb{83.5} & \textsb{96.9}  & \textsb{97.0}   & 90.0  & 29.0  & 36.0 & 64.2 & 67.5 & 72.3  \\
     BYOL-S & 91.1  & \textsb{83.8} & 92.3  & \textsb{97.3}  & \textsb{92.9} & 42.0 & 44.0 & 70.0 & 73.4 & 76.3 \\
     BYOL-S\texttt{++} & \textsb{95.3}  & \textsb{83.9} & 93.8 & \textsb{97.4} & 91.7 & 40.0 & 41.8 & 69.6 & 73.2 & 76.3 \\
     \bottomrule
    \end{NiceTabular}
    \label{tab:pretraining_results_music}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/Table810.tex <==
\begin{table}[h!]
\small
\centering
\vspace{-0.3cm}
\caption{Top-1 accuracy of input window-based variants of BYOL-S on speech-related tasks. All HEAR baselines were achieved using wav2vec2.}
\begin{tabular}{l@{\hspace{20pt}}cccccc@{\hspace{20pt}}c}
\toprule
        \begin{tabular}{@{}l@{}}BYOL-S \\ Window Size (s)\end{tabular} & \rotatebox{90}{CREMA-D} 
        & \rotatebox{90}{LibriCount} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (5h)}} 
        & \rotatebox{90}{\parbox{.25cm}{Speech \\ Commands (all)}} 
        & \rotatebox{90}{\parbox{.25cm}{Vocal \\ Imitations}} 
        & \rotatebox{90}{VoxLingua} 
        & \rotatebox{90}{Average} \\
\midrule
HEAR & 65.6 & 69.2 & 87.9 & 83.8 & 6.8 & \textsb{49.3} & 59.3 \\
\midrule
0.5   & \textsb{66.5} & \textsb{86.0}          & 91.2             & 93.4          & 14.2         & 43.0           & 64.8    \\
0.95  & 65.5          & 83.0          & \textsb{91.9}             & \textsb{94.5} & 14.8         & 44.4          & 65.2     \\
1.425 & 65.7          & 81.0          & 90.0               & 93.1          & \textsb{16.0} & 43.1          & 64.7    \\
2     & 65.6          & 81.8 & \textsb{92.2}    & 93.4          & 14.3         & 47.3 & \textsb{65.8}    \\
\bottomrule
\end{tabular}
\label{tab:audio_win_speech}\vspace{-0.3cm}
\end{table}

\begin{table}[h!]
\small
\centering
\caption{Contribution of the pre-training window size on environment sound-related tasks. Top-1 accuracy was used for each dataset but FSD50K (mAP). HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
\begin{tabular}{l@{\hspace{20pt}}cccc@{\hspace{20pt}}c}
    \toprule
    \begin{tabular}{@{}l@{}}BYOL-S \\ Window Size (s)\end{tabular}  & \rotatebox{90}{Beehive states} & \rotatebox{90}{ESC} & \rotatebox{90}{FSD50K} & \rotatebox{90}{\parbox{.25cm}{Gunshot \\ triangulation}}       & \rotatebox{90}{Average}\\
    \midrule
     HEAR & 53.5$^\sharp$ & 56.1$^\dagger$ & 34.2$^\dagger$ & 86.3$^\sharp$ & 57.5\\ 
     \midrule
     0.5   & \textsb{59.7} & \textsb{83.3} & \textsb{49.5}         & 89.3          & \textsb{70.5}\\
     0.95  & 57.5          & 81.4          &  \textsb{50.0} & \textsb{95.2} & \textsb{71.0}\\
     1.425 & 56.5          & 80.3          & \textsb{49.9}         & 89.3          & 69.0\\
     2     & 53.5          & 81.3          & \textsb{49.6}         & \textsb{95.2} & 69.9 \\
\bottomrule
\end{tabular}
\label{tab:audio_win_env}\vspace{-0.4cm}
\end{table}
\setlength{\tabcolsep}{6pt}

\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
\small
\centering
\caption{Top-1 accuracy of input window-based variants of BYOL-S on music-related tasks. S/M: Speech vs. Music task. HEAR baselines: $\sharp$: CREPE, $\dagger$: wav2vec2.}
\begin{NiceTabular}{l@{\hspace{10pt}}c@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}*{2}{c}@{\hspace{10pt}}c}
\toprule
BYOL-S & \Block{1-1}{\rotate Beijing Opera} & \Block{1-2}{\rotate GTZAN} && \Block{1-2}{\rotate Mridangam} &&  \Block{1-2}{\rotate NSynth (5h)} && \Block{1-2}{\rotate NSynth (50h)} && \rotatebox{90}{Average} \\
% \cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}\cmidrule{9-10}
Window Size (s)  & & Genre & S/M & Stroke & Tonic & Pitch & Chroma & Pitch & Chroma \\
\midrule
HEAR & 92.8$^\sharp$ & 78.0$^\dagger$ & 94.6$^\dagger$ & 94.3$^\dagger$ & 82.8$^\dagger$ & \textsb{87.0}$^\sharp$ & \textsb{92.6}$^\sharp$ & \textsb{90.0}$^\sharp$ & \textsb{95.7}$^\sharp$ & \textsb{89.8} \\
\midrule
 0.5   & \textsb{94.9} & \textsb{83.5} & 96.9 & \textsb{97.3}           &  \textsb{93.0} & 38.2           &  40.6           &  71.2          &  74.5 & 76.7           \\

 0.95  & 93.2          & 82.5 & 96.2 & \textsb{97.3} & \textsb{92.5} & 38.2            & 39.0            & 69.0           & 72.1 & 75.6                 \\
 1.425 & \textsb{94.5}    & \textsb{83.6} &   \textsb{98.5}      & \textsb{97.0}          & \textsb{92.5}    & 35.2            & 37.6           & 67.7          & 71.6 & 75.4                  \\
 2     & 94.1       & \textsb{83.4} &       \textsb{98.5} &  \textsb{97.1}           & 91.9   & 35.8            & 37.4           & 66.2          & 69.2 & 74.8  \\
\bottomrule
\end{NiceTabular}
\label{tab:audio_win_music}\vspace{-0.4cm}
\end{table}
\setlength{\tabcolsep}{6pt}

==> drafts/drafts_table3.tex <==
% \begin{table}[]
% \centering
% \caption{Results on Speech-based Tasks}
% \begin{tabular}{llll}
% \toprule
%                   & BYOL-A & BYOL-S         & BYOL-S++       \\
% \midrule
% CREMA-D            & 0.623  & \textbf{0.664} & \textbf{0.664} \\
% Speech Command 5h  & 0.896  & 0.926          & \textbf{0.932} \\
% Speech Command ALL & 0.924  & 0.943          & \textbf{0.95}  \\
% LibriCount         & 0.788  & 0.786          & \textbf{0.8}   \\
% VoxLingua          & 0.39   & 0.412          & \textbf{0.478} \\
% Vocal Imitation    & 0.137  & 0.151          & \textbf{0.154} \\
% \bottomrule
% \end{tabular}
% \label{results_speech}
% \end{table}

% \begin{table*}[t]
% \hspace{-2.8cm}
%   \begin{tabular}{c|c|c|c|c|c|c}
%     Model Name & CREMA-D & Speech Command 5h & Speech Command ALL & LibriCount & VoxLingua & Vocal Imitation \\
%     \midrule
%      BYOL-A &  0.623 & 0.896 & 0.924 & 0.788 & 0.39 & 0.137    \\
%      BYOL-S &  0.664 & 0.926 & 0.943 & 0.786 & 0.412 & 0.151 \\
%      BYOL-S++ & 0.664 & \textbf{0.932} & \textbf{0.95} & \textbf{0.8} & \textbf{0.478} & \textbf{0.154} \\
%   \end{tabular}
%   \caption{Results on Speech-based Tasks}
%   \label{tab:1}
% \end{table*}

==> drafts/drafts_table4.tex <==
\setlength{\tabcolsep}{1.25pt}
\begin{table*}[t]
    \centering
    \caption{Performance of BYOL-A, BYOL-S and BYOL-S++ variants on speech-based environmental sounds tasks}
    \vspace{2pt}
    \begin{tabular}{cccccccccccc}
    \toprule
            & \rotatebox{90}{Beehive States}  & \rotatebox{90}{Beijing Opera} & \rotatebox{90}{ESC} & \rotatebox{90}{FSD50K} & \rotatebox{90}{Gunshot triangulation} & \rotatebox{90}{Mridangam Stroke} & \rotatebox{90}{Mridangam Tonic} & \multicolumn{2}{c}{\rotatebox{90}{NSynth 5h}} & \multicolumn{2}{c}{\rotatebox{90}{NSynth 50h}} \\
            & & &  & & & & & Pitch & Chroma & Pitch & Chroma \\
    \midrule
     BYOL-A &  0.488          & 0.919          & 0.789          & 0.489          & 0.875          & 0.97           & 0.9            & 0.29          & 0.306         & 0.642        & 0.675  \\
     
     BYOL-S &  \textbf{0.528} & 0.911          & \textbf{0.819} & \textbf{0.499} & \textbf{0.964} & 0.973          & \textbf{0.929} & \textbf{0.42} & \textbf{0.44} & \textbf{0.7} & \textbf{0.734} \\
     
     BYOL-S++ & 0.505         & \textbf{0.953} & 0.8            & 0.494          & 0.929          & \textbf{0.974} & 0.917          & 0.4           & 0.418         & 0.696        & 0.732 \\
     \bottomrule
  \end{tabular}
  
  \label{tab:1}
\end{table*}

==> drafts/drafts_table6.tex <==
\begin{table*}[t]
\hspace{-2.8cm}
  \begin{tabular}{c|c|c|c|c|c|c}
    Model Name & CREMA-D & Speech Command 5h & Speech Command ALL & LibriCount & VoxLingua & Vocal Imitation \\
    \midrule
     BYOL-S, 0.5 sec &  - & 0.912 & 0.934 & 0.806 & 0.43 & 0.142    \\
     BYOL-S, 0.95 sec &  - & 0.919 & 0.945 & 0.803 & 0.444 & 0.148 \\
     BYOL-S,  1.425 sec & - & 0.9 & 0.931 & 0.801 & 0.431 & 0.16 \\
     BYOL-S, 2 sec &  - & 0.922 & 0.934 & 0.818 & 0.473 & 0.143 \\
  \end{tabular}
  \caption{Results on Speech-based Tasks}
  \label{tab:1}
\end{table*}

==> drafts/drafts_table7.tex <==
\begin{table*}[t]
\hspace{-2.8cm}
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    Model Name & Beehive States & Beijing Opera & ESC & FSD50K & Gunshot triangulation & Mridangam Stroke & Mridangam Tonic & \multicolumn{2}{c}{NSynth 5h} & \multicolumn{2}{c}{NSynth 50h} \\
    \midrule
     BYOL-S, 0.5 sec &  0.597 & 0.949 & 0.833 & 0.495 & 0.893 & 0.382 & 0.406 & 0.712 & 0.745 & 0.973 & 0.93  \\
     BYOL-S, 0.95 sec &  0.575 & 0.932 & 0.814 & 0.5 & 0.952 & 0.382 & 0.39 & 0.69 & 0.721 & 0.973  & 0.925\\
     BYOL-S, 1.425 sec &  0.565 & 0.945 & 0.803 & 0.499 & 0.893 & 0.352 & 0.376 & 0.677 & 0.716 & 0.97 & 0.925 \\
     BYOL-S, 2 sec & 0.535 & 0.941 & 0.813 & 0.496 & 0.952 & 0.358 & 0.374 & 0.662 & 0.692 & 0.971 & 0.919 \\
  \end{tabular}
  \caption{Results on Environmental and Instrumental Sounds Tasks}
  \label{tab:1}
\end{table*}

==> drafts/drafts_table8.tex <==
\begin{table*}[t]
\hspace{-2.8cm}
  \begin{tabular}{c|c|c|c|c|c|c}
    Model Name & CREMA-D & Speech Command 5h & Speech Command ALL & LibriCount & VoxLingua & Vocal Imitation \\
    \midrule
     BYOL-S, AudioNTT &  - & 0.926 & 0.943 & 0.786 & 0.412 & 0.151    \\
     BYOL-S, Resnetish34 &  - & 0.832 & 0.889 & 0.77 & 0.358 & 0.148 \\
     BYOL-S,  CLSTM & - & 0.913 & 0.925 & 0.781 & 0.243 & 0.16 \\
     BYOL-S, CvT &  - & 0.92 & 0.931 & 0.848 & 0.37 & 0.162 \\
  \end{tabular}
  \caption{Results on Speech-based Tasks}
  \label{tab:1}
\end{table*}

==> drafts/drafts_table9.tex <==
\begin{table*}[t]
\hspace{-2.8cm}
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    Model Name & Beehive States & Beijing Opera & ESC & FSD50K & Gunshot triangulation & Mridangam Stroke & Mridangam Tonic & \multicolumn{2}{c}{NSynth 5h} & \multicolumn{2}{c}{NSynth 50h} \\
    \midrule
     BYOL-S &  0.528 & 0.911 & 0.819 & 0.499 & 0.964 & 0.42 & 0.44 & 0.7 & 0.734 & 0.973 & 0.929  \\
     BYOL-S/Resnetish-34 &  0.528 & 0.924 & 0.715 & 0.433 & 0.863 & 0.206 & 0.224 & 0.449 & 0.474 & 0.961  & 0.887\\
     BYOL-S/CLSTM &  0.514 & 0.907 & 0.739 & 0.394 & 0.869 & 0.286 & 0.32 & 0.576 & 0.605 & 0.967 & 0.897 \\
     BYOL-S/CvT & - & 0.962 & 0.799 & 0.483 & 0.893 & 0.53 & 0.552 & 0.761 & 0.805 & 0.975 & 0.94 \\
  \end{tabular}
  \caption{Results on Environmental and Instrumental Sounds Tasks}
  \label{tab:1}
\end{table*}



==> other/CHANGES <==
v1.30 (2022-02-09):

  * jmlrutils.sty:

    - fixed counter name in lemma definition when cleveref option on

v1.29 (2022-01-29):

  * jmlr.cls:

    - added cleveref option

    - fixed draft option

    - bug fix #168: Float-only last pages not counted for page numbering
       https://www.dickimaw-books.com/bugtracker.php?key=168

  * jmlrutils.sty:

    - added cleveref option

    - added \jmlralgorule

    - added \jmlrminsubcaptionwidth

  * jmlrbook.cls:

    - obsoleted (https://www.dickimaw-books.com/faq.php?itemlabel=latex20201009)
      Production editors will need to set the first page number
      of each article manually.

v1.28 (2020-09-21):

  * jmlr.cls:

   Bug fixes: 

    - fixed twoside option (which should be the default)

    - \thanks now uses mpfootnote instead of footnote counter
      with matching \footnotemark and \footnotetext optional
      arguments.

v1.27 (2020-03-26):

  * jmlrutils.sty:

    Bug fix: subfigure and subtable references were producing
    extraneous text (added check for LaTeX kernel version)

v1.26 (2020-01-31):

  * jmlr.cls:

    - removed \vbox from \@jmlrmaketitle to allow for extremely long
      author/affiliation list. Added \ignorespaces before \@author
      to allow for spacing the contents in the code for clarity
      at the start of a long author list.

v1.25 (2020-01-17):

  * jmlr.cls: 

    - Added check for graphics.sty 2019/07/01 (which now detokenizes
      filename)

  * jmlrutils.sty:

    - Added \proofname

v1.24 (2017-08-01):

  * moved non-class related code into new package jmlrutils.sty

  * fixed bug in \includeteximage

v1.23 (2017-03-09):

  * added pmlr class option

v1.22 (2015-04-11):

  * added oneside and twoside class options

v1.21 (2015-02-24):

  * jmlr.cls

    - added check for jmlr2e and pseudocode

    - fixed bug in \thanks to fix footnote marker issue if there's
      more than one \thanks

  * jmlrbook.cls

    - added \nopagebreak after \@editorialteam

v1.20 (2014-10-15):

  * jmlrbook.cls

    - added \jmlrprefaceheader, \jmlrlocation

v1.19 (2014-09-29):

  * jmlrbook.cls

    - changed \chapter* to \chapter in preface environment

v1.18 (2013-10-17):

  * jmlrbook.cls

    - patched to work with auxhook

    - added draft and final options

    - add \booklinebreak

  * jmlr.cls

    - Added calc and etoolbox as required packages

    - Added draft and final options and removed \ds@draft

    - Added starred version of \newtheorem

    - Added \theorembodyfont, \theoremheaderfont, \theorempostheader
      and \theoremsep

v1.17 (2012-05-30):

  * jmlr.cls

    - added \titletag

    - added warnings if obsolete font commands (such as \bf) used

  * jmlrbook.cls

    - added 'articlet' page style

    - \importarticle sets title page style to articlet

    - \importpaper disables \jmlryear, \jmlrworkshop, \jmlrvolume
      and \jmlrissue

    - html title page uses jmlrvolume instead of volume

    - added optional argument to \logo

v1.16 (2012-05-15):

  * jmlr.cls

    - added \@post@hyperref hook

  * jmlrbook.cls

    - added code to deal with \c@lenddoca clash

v1.15 (2012-05-12):

  * jmlrbook.cls

    - added 'algocf' and 'definition' counters to reset list in
      \zeroextracounters

    - added \theHalgocf

    - removed dependence on \ps@headings in \ps@jmlrbook

    - added \markleft

v1.14 (2012-04-24):

  * jmlrbook.cls

    - modified \jmlrwritepdfinfo to write book author and title
      information to aux file
    - fixed bug in fetching time zone information

v1.13 (2012-02-25):

  * jmlrbook.cls

    - added pdfxa option
    - added \jmlrwritepdfinfo
    - changed preface environment to use \chapter* instead of \chapter

  * jmlr.cls

    - added \@pre@hyperref hook

v1.12 (2012-01-05):

  * jmlr.cls

    - removed prehyperref package option.

    - renamed \jmlr@prehyperref to \jmlrprehyperref

    - added tabularx to list of problem packages.

    - provided default value of \@shortitle

    - added \titlebreak

    - added optional argument to \Name
      (\jmlrauthors now redefines \@jmlr@authors instead of
      \@jmlrauthors)

    - added chapter number to \theHsection to ensure unique
      hyperlinks in book

  * jmlrbook.cls

    - Moved loading setspace and fink before jmlr.cls loaded

    - changed \thechapter to \theHchapter in definition of
      \theHalgorithm etc

    - added \theHfootnote, \theHtable, \theHfigure

    - in \importpubpaper etc, changed \@shortitle to \@title in toc

  * makejmlrbook v0.31

    - footnotes in abstract files changed to in-line parentheses.

    - --batchtex option now also passes "-interaction=batchmode" to
      htlatex

    - added debugging option --noexecute

v1.11 (2011-03-24):

  * jmlr.cls

    - fixed typo: WC\&P -> W\&CP

    - added \jmlrabbrnamelist (used by makejmlrbook)

  * jmlrbook.cls

    - now requires fink package

    - added preface environment and \prefacename

    - added algorithm2e old commands (in case some authors are using
      an older version).

  * makejmlrbook (v0.3):

    - added changes made by Olivier Chapelle to add JMLR menu on the
      left side of the page and use description environment for each
      paper of the TOC.

    - added --extractpreface option

    - set hyperref draft mode for abstract only html pages.

    - abstract html source files now input original aux files to allow
      for citations.

v1.10 (2011-01-05):

  jmlr.cls

  * now loads xkeyval

  * now loads hyperref (instead of jmlrbook loading it)

  * added class option prehyperref={stuff to do before hyperref loaded}

  * added class option tablecaption=<position> (where <position> can
    either be top or bottom).

  * fixed 10pt, 11pt and 12pt class options, which weren't having
    any effect.

  * modified \thanks to ensure hyperlink works correctly.

  * added \mdseries to definition of \addr.

  * added \startpage (used by jmlrmakebook).

  * modified \artpart and \bookpart to correct bookmark level number

  jmlrbook.cls

  * code loading hyperref moved to jmlr.cls

  * added 10pt, 11pt and 12pt class options.

  * Removed redundant redefinition of \@bookpart

  makejmlrbook (v0.2):

  * Uses \startpage to set initial page number for stand-alone 
    articles.

  * Makes subdirectories in html directory for each article.

  * copies any image files generated by tex4ht into html directory.

  * added time stamp at the end of each of the generated html file.

v1.09 (2010-12-01):

  jmlr.cls

  * now loads article.cls instead of scrartcl.cls

  * Fixed sub-captions so that they don't exceed the width of the
    sub-figure/table to which they refer.

  * added \nametag, \reprint, \algocfconts, \theHsubfigure,
    \booktocpreamble, \@partapp.

  * Made \objectref robust

  jmlrbook.cls

  * Reset start and end document hook to avoid problems caused by
    defining duplicate commands.

  * Moved redefinition of \jmlrpremaketitlehook outside of import
    macros.

  * Moved \refstepcounter from \jmlrmaketitlehook to
    \jmlrpremaketitlehook

  * Added \jmlrimporthook

  * Added \label to \jmlrmaketitlehook

v1.08 (2010-07-27):

  * Fixed \thanks so that the footnote symbol is raised and isn't
    followed by a full stop.

v1.07 (2010-06-30):

  * Added check for two column

v1.06 (2010-06-17):

  jmlr.cls

  * Added tablecaptiontop and tablecaptionbottom class options

v1.05:

  jmlrbook.cls

  * Added \productioneditors

v1.04:

  * Added Perl script makejmlrbook

  jmlrbook.cls

  * Added patch to fix references in print mode

  * Added code to work with makejmlrbook

  jmlr.cls

  * Added code to work with makejmlrbook

v1.03:
  jmlrbook.cls

  * Added patch to combnat

  jmlr.cls

  * Added \editors, \editorname and \editorsname

v1.02:
  jmlrbook.cls:

  * Added \issue

  jmlr.cls

  * Added \jmlrissue

v1.01 :

  jmlrbook.cls: 

  * added \importpaper

  * added \titlebody, \SetTitleElement and \IfTitleElement to 
    make it easier to customise the front page of the book.

  jmlr.cls:

  * fixed the last page anchor.

v1.0 : Initial release

